Abstract Syntax Tree for Programming Language Understanding and Representation: How Far Are We?

Programming language understanding and representation (a.k.a code representation learning) has always been a hot and challenging task in software engineering. It aims to apply deep learning techniques to produce numerical representations of the source code features while preserving its semantics. These representations can be used for facilitating subsequent code-related tasks. The abstract syntax tree (AST), a fundamental code feature, illustrates the syntactic information of the source code and has been widely used in code representation learning. However, there is still a lack of systematic and quantitative evaluation of how well AST-based code representation facilitates subsequent code-related tasks. In this paper, we first conduct a comprehensive empirical study to explore the effectiveness of the AST-based code representation in facilitating follow-up code-related tasks. To do so, we compare the performance of models trained with code token sequence (Token for short) based code representation and AST-based code representation on three popular types of code-related tasks. Surprisingly, the overall quantitative statistical results demonstrate that models trained with AST-based code representation consistently perform worse across all three tasks compared to models trained with Token-based code representation. Our further quantitative analysis reveals that models trained with AST-based code representation outperform models trained with Token-based code representation in certain subsets of samples across all three tasks. We also conduct comprehensive experiments to evaluate and reveal the impact of the choice of AST parsing/preprocessing/encoding methods on AST-based code representation and subsequent code-related tasks. Our study provides future researchers with detailed guidance on how to select solutions at each stage to fully exploit AST.

==> tables/RQ2-clone.tex <==
\begin{table}[htbp]
    \caption{Effectiveness of AST in promoting code clone detection. }
    \label{table:RQ2-clone}
    \centering  
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
        %\Xhline{2pt}
        \toprule
        
        Model & Input & Recall & Precision & $F_1$ \\
        
        %\hline
        \midrule
        
        \multirow{4}{*}{BiLSTM}& Token & \textbf{88.92} & \textbf{90.35} & \textbf{89.62} \\
        {} & SBT & 73.06 & 78.68 & 75.77 \\
        {} & SBT w/o Token & 40.91 & 42.71 & 41.79 \\
        {} & Token + SBT w/o Token & 86.06 & 90.05 & 88.01 \\
        
        %\hline
        \midrule

        \multirow{4}{*}{Transformer}& Token & \textbf{93.80} & 93.15 & \textbf{93.74} \\
        {} & SBT & 92.57 & 91.06 & 91.81 \\
        {} & SBT w/o Token & 68.47 & 58.40 & 63.03 \\
        {} & Token + SBT w/o Token & 91.39 & \textbf{93.75} & 92.55 \\

        \bottomrule
        %\Xhline{2pt}
    \end{tabular}
    }
\end{table}

==> tables/RQ3-clone.tex <==
\begin{table}[htbp]
    \caption{Performance of different AST parsing methods in code clone detection task}
    \label{tab:RQ3-clone}
    \centering  
    \resizebox{\linewidth}{!}{
        \begin{tabular}{c|cccc}
        \Xhline{2pt}
        {} & AST parser & Recall & Precision & F1 \\
        
        \hline
        
        \multirow{4}{*}{SBT+Bi-LSTM}& JDT & \textbf{73.06} & 78.68 & \textbf{75.77} \\
        {} & srcML & 69.77 & \textbf{80.39} & 74.70 \\
        {} & ANTLR & 71.59 & 80.11 & 75.61 \\
        {} & Tree-sitter & 72.56 & 79.00 & 75.64 \\
        
        \hline
        
        \multirow{4}{*}{AST+Tree-LSTM}& JDT & 84.25 & \textbf{92.18} & \textbf{88.04} \\
        {} & srcML & 78.13 & 82.87 & 80.43 \\
        {} & ANTLR & \textbf{87.06} & 84.04 & 85.52 \\
        {} & Tree-sitter & 84.76 & 88.36 & 86.52 \\
        
        \Xhline{2pt}
        \end{tabular}
    }
\end{table}

==> tables/RQ3-search.tex <==
\begin{table}[htbp]
    \caption{Performance of different AST parsing methods in code search task}
    \label{tab:RQ3-search}
    \centering  
    \resizebox{\linewidth}{!}{
        \begin{tabular}{c|ccccc}
        \Xhline{2pt}
        Model & Input Type & SR@1 & SR@5 & SR@10 & MRR \\ 
        
        \hline
        
        \multirow{4}{*}{SBT+BiLSTM}& JDT & 0.1720 & \textbf{0.4052} & \textbf{0.5276} & \textbf{0.2827} \\
        {} & srcML & 0.1395 & 0.3023 & 0.3604 & 0.2254 \\  
        {} & ANTLR & 0.1279 & 0.2093 & 0.2674 & 0.1791 \\  
        {} & Tree-sitter & \textbf{0.1744} & 0.3605 & 0.4419 & 0.2732 \\ 
        
        \hline
        
        \multirow{4}{*}{AST+Tree-LSTM}& JDT & \textbf{0.0906} & \textbf{0.2076} & \textbf{0.2660} & \textbf{0.1524} \\
        {} & srcML & 0.0556 & 0.1784 & 0.2485 & 0.1181 \\  
        {} & ANTLR & 0.0760 & 0.1520 & 0.2251 & 0.1226 \\  
        {} & Tree-sitter & 0.0760 & 0.1784 & 0.2193 & 0.1268 \\ 
        
        \Xhline{2pt}
        \end{tabular}
    }
\end{table}

==> tables/RQ3-summarization.tex <==
\begin{table}[htbp]
    \caption{Performance of different AST parsing methods in code summarization task}
    \label{tab:RQ3-summarization}
    \centering  
    \resizebox{\linewidth}{!}{
        \begin{tabular}{c|cccc}
            \Xhline{2pt}
            {} & Input & BLEU & METEOR & ROUGE-L \\
            
            \hline
            
            \multirow{4}{*}{SBT+BiLSTM}& JDT & \textbf{9.021} & \textbf{4.540} & 16.45 \\
            {} & srcML & 8.672 & 4.021 & \textbf{17.03} \\  
            {} & ANTLR & 7.689 & 3.353 & 13.48 \\  
            {} & Tree-sitter & 8.663 & 4.333 & 15.99 \\ 
            
            \hline
            
            \multirow{4}{*}{AST+Tree-LSTM}& JDT & \textbf{9.781} & \textbf{5.317} & \textbf{18.54} \\
            {} & srcML & 9.578 & 3.516 & 18.28 \\  
            {} & ANTLR & 9.372 & 3.425 & 17.79 \\  
            {} & Tree-sitter & 9.279 & 3.521 & 17.97 \\ 
            
            \Xhline{2pt}
        \end{tabular}
    }
\end{table}
